Partial Large Kernel CNNs for Efficient Super-Resolution

Recently, in the super-resolution (SR) domain, transformers have outperformed CNNs with fewer FLOPs and fewer parameters since they can deal with long-range dependency and adaptively adjust weights based on instance. In this paper, we demonstrate that CNNs, although less focused on in the current SR domain, surpass Transformers in direct efficiency measures. By incorporating the advantages of Transformers into CNNs, we aim to achieve both computational efficiency and enhanced performance. However, using a large kernel in the SR domain, which mainly processes large images, incurs a large computational overhead. To overcome this, we propose novel approaches to employing the large kernel, which can reduce latency by 86\% compared to the naive large kernel, and leverage an Element-wise Attention module to imitate instance-dependent weights. As a result, we introduce Partial Large Kernel CNNs for Efficient Super-Resolution (PLKSR), which achieves state-of-the-art performance on four datasets at a scale of $\times$4, with reductions of 68.1\% in latency and 80.2\% in maximum GPU memory occupancy compared to SRFormer-light.

==> Table/LargeDF2KResults.tex <==
\begin{table*}[h]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|c|ccc|ccccc@{}}
\toprule
Methods        & Scale                        & Latency{[}ms{]} & \#VP{[}Mb{]} & \#Params{[}K{]} & Set5                           & Set14                         & BSD100                         & Urban100                     & Manga109     \\ \midrule
OmniSR         &                              & 64.73 & 669.67 & 772   & 38.22/0.9613 & 33.98/0.9210 & 32.36/0.9020 & 33.05/0.9363 & 39.28/0.9784 \\
CRAFT          &                              & 106.00 & 644.30 & 737   & 38.23/0.9615 & 33.92/0.9211 & 32.33/0.9016 & 32.86/0.9343 & 39.39/0.9786 \\
\textbf{Ours-L}  & \multirow{-3}{*}{$\times$2}& 55.84 & 747.65 & 392   &  &  &  &  & \\ \midrule

OmniSR         &                              & 24.01 & 307.82 & 780   & 34.70/0.9294 & 30.57/0.8469 & 29.28/0.8094 & 28.84/0.8656 & 34.22/0.9487 \\
CRAFT          &                              & 43.49 & 296.13 & 744   & 34.71/0.9295 & 30.61/0.8469 & 29.24/0.8093 & 28.77/0.8635 & 34.29/0.9491 \\
\textbf{Ours-L}  & \multirow{-3}{*}{$\times$3}& 17.50 & 383.78 & 393        &  &  &  &  & \\ \midrule

OmniSR         &                              & 23.91 & 258.03 & 792   & 32.49/0.8988 & 28.78/0.7859 & 27.71/0.7415 & 26.64/0.8018 & 31.02/0.9151 \\
CRAFT          &                              & 41.40 & 231.50 & 753   & 32.52/0.8989 & 28.85/0.7872 & 27.72/0.7418 & 26.56/0.7995 & 31.18/0.9168 \\
\textbf{Ours-L}  & \multirow{-3}{*}{$\times$4}& 9.94 & 278.54 & 395             &  &  &  &  & \\ \bottomrule
\end{tabular}
}
\caption{Comparisons of Classic SR networks trained on DIV2K Dataset.}\label{tab:LSDIR}
\end{table*}


==> Table/MobileLatency.tex <==
\begin{table}[]
\caption{Mobile Latency Comparison. All latencies are measured using the CoreML library. $^{\dagger}$ means that since their
codes were unavailable, we re-implemented them. Implementation detail은 supplementary 참조.}\label{tab:mobilelatency}
\vspace{-0.4cm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|cc|c@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Latency(iPhone12, ms)} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Performance\\ (PSNR, B100$\times$2)\end{tabular}} \\ \cmidrule(lr){2-3}
 & $X\in\mathbb{R}^{3\times96\times96}$ & $X\in\mathbb{R}^{3\times360\times640}$ &  \\ \midrule
EDSR~\cite{EDSR} & 83.50 &  & 32.32 \\
SwinIR-Light~\cite{SwinIR} &  &  & 32.31 \\
ELAN-Light~\cite{ELAN} &  &  & 32.30 \\
CRAFT~\cite{CRAFT} &  &  & 32.33 \\
SRFormer-Light~\cite{SRFormer} &  &  & 32.36 \\
DITN$^{\dagger}$~\cite{DITN} &  &  & 32.32 \\
PLKSR & 474.04 &  & 32.36 \\ \bottomrule
\end{tabular}
}
\end{table}


==> checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}

  
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}

  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{contribution}.}
    
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{conclusion}.}
    
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{intro}.}
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
    
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{assumptions}.}
    
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:derivation}.}
    
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is in the supplemental material. The data can be refered to Section~\ref{dataset}}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerYes{See Section~\ref{dataset} and~\ref{imple_detail}.}
    
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
    
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{imple_detail}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}

  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{dataset}.}
    
  \item Did you mention the license of the assets?
    \answerNA{}
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
    
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
    
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
    
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
    
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
